Numerical Discretization Methods for Linear Quadratic Control Problems with Time Delays

This paper presents the numerical discretization methods of the continuous-time linear-quadratic optimal control problems (LQ-OCPs) with time delays. We describe the weight matrices of the LQ-OCPs as differential equations systems, allowing us to derive the discrete equivalent of the continuous-time LQ-OCPs. Three numerical methods are introduced for solving proposed differential equations systems: 1) the ordinary differential equation (ODE) method, 2) the matrix exponential method, and 3) the step-doubling method. We implement a continuous-time model predictive control (CT-MPC) on a simulated cement mill system, and the objective function of the CT-MPC is discretized using the proposed LQ discretization scheme. The closed-loop results indicate that the CT-MPC successfully stabilizes and controls the simulated cement mill system, ensuring the viability and effectiveness of LQ discretization.

==> tex/Conclusions_ZHAZ.tex <==
\section{Conclusions}
\label{sec:Conclusions}
In this paper, we have introduced the delay-free discrete-time state space representations of continuous-time linear systems with time delays and LQ discretization for continuous-time LQ-OCPs with time delays. We described the LQ discretization as differential equations systems in our propositions and introduced three numerical methods for solving them. In the numerical experiment, we developed a model predictive controller using LQ discretization and proposed numerical methods for a simulated cement mill system. The experiment result indicates that the LQ discretization-based MPC can successfully stablize and control the simulated cement mill system.

==> tex/Introduction_ZHAZ.tex <==
\section{Introduction}
Time delays are pervasive in numerous industrial processes, shaping control systems' trajectories by not solely relying on the present state but also integrating their history. These delays can significantly influence the robustness and performance of the control systems \citep{LEE1995TimeDelaySystems,Gu2003StabilityOT}. Linear-quadratic (LQ) optimal control is considered a fundamental but essential problem in optimal control theory. LQ optimal control problems (LQ-OCPs) described by time-delay systems find extensive practical applications due to the prevalence of time delays, such as chemical reactors, power plants, and transportation systems. In practical applications, the necessity arises to discretize continuous-time LQ-OCPs for digital implementation. In addition, LQ-OCPs play an essential role in other advanced control algorithms, such as linear-quadratic Gaussian (LQG) and model predictive control (MPC) \citep{BAGTERPJORGENSEN2012187,John2013EfficientImplementationofRiccati}. Therefore, developing discretization techniques for LQ-OCPs with time delays becomes both requisite and pivotal. The discretization and numerical methods of time-delay systems and optimal control problems are well-studied, and the relevant literature is vast \citep{Pooja2023ASystematicReview,Cullum1969DiscreteApproximationstoContinuoustimeOCP,Cullum1971AnExplicitProcedure,Han2010ConvergenceofDiscretetime,BAGTERPJORGENSEN2012187,pechlivanidou2022zero,Alt2011RegularizationAD}. However, it is different for the discretization of continuous-time LQ-OCPs, especially for the time-delay case. 

\cite{franklin1990DigitalControl} introduced discretization techniques for continuous-time systems with integer and fractional delays. \cite{kassas2006discretization} further investigated delayed continuous-time systems and provided the discrete-equivalent state space systems. The continuous-time LQ-OCPs can be converted into discrete-time by implementing zero-order hold (ZOH) discretization on the system inputs and states \citep{Hendricks2008LCD}. \cite{Karl1970IntroToStoContTheory} and~\cite{astrom2011computer} described the discrete-time approximation of continuous-time LQ-OCPs, where the cost equivalent is obtained by extending the objective function of the continuous-time LQ-OCP. It subsequently leads to the analytic expressions of desired discrete weighting matrices. \cite{franklin1990DigitalControl} pointed out the desired discrete weighting matrices can be solved using the matrix exponential method \citep{Moler1978NineteenDubiousWays,ExponentialIntegrators2011Higham}. Compared with the ZOH discretization-based method, the second discretization method provides a better approximation. However, the two discretization methods only consider continuous-time LQ-OCPs without time delays, and only limited research exists for the discretization of LQ-OCPs governed by time-delay systems. 
% In addition, 
% Continuous-time stochastic LQ-OCPs can be valuable in many scenarios, e.g., conditional Value-at-Risk optimization problems \citep{Rockafellar2001Conditionalvalueatrisk,CAPOLEI2015214}. 
% %
\cite{Karl1970IntroToStoContTheory} and~\cite{astrom2011computer} introduced the analytic expressions of continuous-time stochastic LQ-OCPs' objective function and its expectation. However, the discretization for continuous-time stochastic LQ-OCPs with time delays has not been addressed in the literature. 

The key problems that we address in this paper: 1) delay-free state space representations of linear time-delay systems, 2) formulation of differential equations systems for deterministic and stochastic LQ discretization with time delays, and 3) numerical methods for solving resulting systems of differential equations.
% \begin{itemize}
%     \item [1.]  Delay-free state space representations of linear time-delay systems
%     \item [2.] Formulation of differential equations systems for deterministic and stochastic LQ discretization with time delays
%     \item [3.] Numerical methods for solving resulting systems of differential equations 
% \end{itemize}
Section~\ref{sec:LinearQuadraticOptimalControlProblems} introduces delay-free discrete-time state space representations of linear time-delay systems and deterministic and stochastic LQ-OCPs with time delays. We propose differential equations systems for the discretization of LQ-OCPs with time delays. Section~\ref{sec:NumericalMethods} describes three numerical methods for solving proposed differential equation systems. We test the LQ discretization and proposed numerical methods by a numerical experiment in Section~\ref{sec:NumericalExperiments} and give the conclusions in Section~\ref{sec:Conclusions}.
%
\section{Linear-Quadratic Optimal Control Problems}
\label{sec:LinearQuadraticOptimalControlProblems}
This section introduces delay-free representations of time-delay systems and describes differential equations systems for LQ discretization.
\subsection{Certainty equivalent LQ for time-delay systems}
Consider a SISO continuous-time linear system
\begin{subequations}
\label{eq:Deterministic-ContinuousTimeDelayStateSpace}% 
\begin{align} 
    \dot x(t) &= A_c x(t) + B_c u(t - \tau), \\ 
    z(t) &= C_c x(t) + D_c u(t - \tau),
\end{align} 
\end{subequations} 
where $x$ is the state, $u$ is the input and $\tau \in \mathbb{R}^{+}_0$ is the time delay.
% where $x \in \mathbb{R}^{n_x \times 1}$ is the states and $u$ is the input. The system matrices $A_c \in \mathbb{R}^{n_x \times n_x}$, $B_c \in \mathbb{R}^{n_x \times 1}$, $C_c \in \mathbb{R}^{1 \times n_x}$, $D_c \in \mathbb{R}^{1 \times 1}$ and the time delay $\tau \in \mathbb{R}^{+}_0$.

Define the sampling time $T_s$ and piece-wise constant input $u(t) = u_k$ for $t_k \leq t < t_{k+1}$. The corresponding delay-free discrete-time state space model of~\eqref{eq:Deterministic-ContinuousTimeDelayStateSpace} is
\begin{subequations}
\begin{align}
    \overbrace{ \left [
                    \begin{array}{c}
                        x_{k+1} \\ \hdashline[2pt/2pt]
                        u_{o,k+1}
                    \end{array}  \right]  }^{=\Tilde{x}_{k+1}} 
    &= \overbrace{ 
         \left[
            \begin{array}{c;{2pt/2pt}c}
                A & B_{o,1} \\ \hdashline[2pt/2pt]
                0 & I_A
            \end{array}
         \right] }^{=\Tilde{A}}
        \overbrace{ \left [
                    \begin{array}{c}
                        x_k \\ \hdashline[2pt/2pt]
                        u_{o,k}
                    \end{array}  \right]  }^{=\Tilde{x}_{k}}
        + 
        \overbrace{
             \left[
                \begin{array}{c}
                    B_{o,2} \\ \hdashline[2pt/2pt]
                    I_B
                \end{array}
             \right] }^{=\Tilde{B}} u_k
        , \\ 
    z_k &= \overbrace{
            \left[
                \begin{array}{c;{2pt/2pt}c}
                    C_c & D_{o,1}
                \end{array}
             \right]
            }^{=\Tilde{C}} \Tilde{x}_k + 
            \overbrace{D_{o,2}}^{=\Tilde{D}} u_k,
\end{align} \label{eq:Deterministic-DiscreteTimeDelayStateSpaceSISO}%
\end{subequations}
where $u_{o,k} = [u_{k-m}; u_{k-m+1}; \ldots; u_{k-1}]$ is the historical inputs. $l =\tau/T_s$ is the time delay constant. $m \in \mathbb{Z}^+_0$ and $0 \leq v < 1$ are the integer and fractional time delay constants with $l = m-v$. $I_A$ and $I_B$ are two constant matrices
\begin{equation} 
I_A = 
    \begin{bmatrix}
        0 & I & \ldots & 0 \\
        \vdots & \vdots & \ddots & \vdots \\
        0 & 0 & \ldots & I \\
        0 & 0 & \ldots & 0 
    \end{bmatrix},
\qquad \qquad  
I_B = 
    \begin{bmatrix}
        0 \\ \vdots \\ 0 \\  I 
    \end{bmatrix}.
\label{eq:IAandIB}
\end{equation}
%
The system matrices $B_{o,1}$, $B_{o,2}$, $D_{o,1}$ and $D_{o,2}$ are
\begin{subequations} \label{eq:SystemMatricesOfDelayFreePresentationSISO} %
\begin{alignat}{3} 
    & B_o = B_1 + B_2, \quad &&
    D_o = D_c e_{m+1}^{m+1},               
    \\
    & B_{o,1} = B_o(:, 1:end-n_u), \: && 
    B_{o,2} = B_o(:, m n_u:end), 
    \\
    & D_{o,1} = D_o(:, 1:end-n_u), && 
    D_{o,2} = D_o(:, m n_u:end),
\end{alignat} 
%
where $e_n^k \in \mathbb{R}^{ n_u \times k n_u }$ is a vector and $e_n^k(:, (k-n)n_u: (k-n+1) n_u)$ = $I$ for $n=1,\ldots, k$, such that $ e_n^k = \begin{bmatrix} 0 & \cdots & I & \cdots & 0 \end{bmatrix}$.
\end{subequations}
% It is defined as 
% \begin{equation}
%     e_n^k = \begin{bmatrix}
%         0 & \cdots & I & \cdots & 0
%     \end{bmatrix},
%     \qquad \text{for} \: \: \: n = 1, \ldots, k.
% \label{eq:e_n^kSISO}
% \end{equation}

%% %%%%%%%%%%%%%%%%%%%%%%%%
% \begin{prop} 
% % [Discretization of the time-delay system (SISO)] 
% \label{prop:DiscretizationofSISOTimeDelaySystem}
% The system of differential equations
% \begin{subequations}
% \label{eq:SISOTimeDelaySystem:MatrixODEsystem}
% \begin{alignat}{3}
%     \dot A(t) &= A_c A(t), \qquad && A(0) = I, \\
%     \dot A_v(t) &= v A_c A_v(t), \qquad && A_v(0) = I, \\ 
%     \dot B_1(t) &= \left(A(t) - vA_v(t) \right)B_{1c}, \qquad && B_1(0) = 0, \\
%     \dot B_2(t) &= vA_v(t)B_{2c}, \qquad && B_2(0) = 0,
% \end{alignat}
% where 
% \begin{equation}
%     B_{1c} = B_c e_{m+1}^{m+1}, \qquad 
%     B_{2c} = B_c e_{m}^{m+1},
% \label{eq:B1candB2cSISOCase}
% \end{equation}
% \end{subequations}
% may be used to compute ($A = A(T_s)$, $B_o=B_1(T_s)+B_2(T_s)$) for the discretization of the SISO time-delay system.
% % {\flushright \hfill $\blacksquare$}
% \end{prop}

% \begin{proposition}[Discretization of the time-delay system (SISO)] 
% The system of differential equations
% \label{prop:DiscretizationofSISOTimeDelaySystem}
% \begin{subequations}
% \label{eq:SISOTimeDelaySystem:MatrixODEsystem}
% \begin{alignat}{3}
%     \dot A(t) &= A_c A(t), \qquad && A(0) = I, \\
%     \dot A_v(t) &= v A_c A_v(t), \qquad && A_v(0) = I, \\ 
%     \dot B_1(t) &= \left(A(t) - vA_v(t) \right)B_{1c}, \qquad && B_1(0) = 0, \\
%     \dot B_2(t) &= vA_v(t)B_{2c}, \qquad && B_2(0) = 0,
% \end{alignat}
% where 
% \begin{equation}
%     B_{1c} = B_c e_{m+1}^{m+1}, \qquad 
%     B_{2c} = B_c e_{m}^{m+1},
% \label{eq:B1candB2cSISOCase}
% \end{equation}
% \end{subequations}
% may be used to compute ($A = A(T_s)$, $B_o=B_1(T_s)+B_2(T_s)$). 
% {\flushright \hfill $\blacksquare$}
% \end{proposition}
%% %%%%%%%%%%%%%%%%%%%%%%%%
Then we consider a MIMO system consists of $n_z \times n_u$ SISO time-delay systems described in~\eqref{eq:Deterministic-ContinuousTimeDelayStateSpace}. The continuous-time system from j$^{th}$ input to i$^{th}$ output is
\begin{subequations}
\label{eq:Deterministic-ContinuousTimeDelayStateSpaceMIMO}
    \begin{align} 
        \dot x_{ij}(t) &= A_{c,ij} x_{ij}(t) + B_{c,ij} u_j(t - \tau_{ij}), \\ 
        z_{i}(t) &= C_{c,ij} x_{ij}(t) + D_{c,ij} u_j(t - \tau_{ij}),
    \end{align}
\end{subequations}
where $A_{c,ij}$, $B_{c,ij}$, $C_{c,ij}$ and $D_{c,ij}$ are identical to the SISO case~\eqref{eq:Deterministic-ContinuousTimeDelayStateSpace} for $i=1,2,\ldots,n_z$ and $j = 1,2,\ldots, n_u$. $x_{ij}$ is the state and $\tau_{ij}$ is the time delay. Denote that $l_{ij}$, $m_{ij}$ and $v_{ij}$ are corresponding time delay constants.

By stacking SISO system matrices, we have
\begin{subequations}
    \begin{equation}
        A_c = \begin{bmatrix}
        A_{c,11} &  &  &\\
        & A_{c,21} & & \\
        & & \ddots & \\
        & & & A_{c,n_z n_u} 
    \end{bmatrix},
    \:
    B_c = \begin{bmatrix}
            \bar{B}_{c,11} \\
            \bar{B}_{c,21} \\
            \vdots \\
            \bar{B}_{c,n_z n_u}
        \end{bmatrix},
    \end{equation}
% and 
    \begin{equation}
        C_c = \begin{bmatrix}
       \bar{C}_{c,1} \\ \bar C_{c,2} \\ \vdots \\ \bar{C}_{c, n_u}
    \end{bmatrix}^T,
    D_c = \begin{bmatrix}
        D_{c,11} & D_{c,12} & \cdots & D_{c, 1 n_u} \\
        D_{c,21} & D_{c,22} & \cdots & D_{c, 2 n_u} \\
        \vdots & \vdots & \ddots & \vdots \\ 
        D_{c,n_z 1} & D_{c,n_z 2} & \cdots & D_{c, n_z n_u}
    \end{bmatrix},
    \end{equation}
\end{subequations}
where 
\begin{equation}
    \bar{B}_{c,ij} = B_{c,ij} e_j, \: 
    \bar{C}_{c,j} = \text{diag} \left(\left[ C_{c, 1j}, C_{c,2j}, \ldots, C_{c,n_zj} \right] \right)^T,
\end{equation}
and $e_j$ = $\left[0 \: \cdots \: 1 \: \cdots \: 0 \right]$ is a vector with $e_j(j) = 1$ for $j = 1,2,\cdots, n_u$. The corresponding system states $x$ = $\left[  x_{11} ; x_{21}; \cdots; x_{n_z n_u} \right]$, the inputs $u$=$\left[ u_1; u_2 ; \cdots;u_{n_u} \right]$ and the time delays $\tau$ = $\left[\tau_{11} ; \tau_{21}; \cdots; \tau_{n_z n_u} \right]$. We then define an integer time delay constant vector $m$ and a fractional time delay constant matrix $V$ as
\begin{equation}
    m = \begin{bmatrix}
        m_{11} \\ m_{21} \\ \vdots \\ m_{n_zn_u}
    \end{bmatrix},
    \quad 
    V = \text{diag} \left( \left[ V_{11}, V_{21}, \cdots, V_{n_z n_u} \right] \right),
\end{equation}
where $V_{ij} = v_{ij} I_{ij}$ and $I_{ij} \in \mathbb{R}^{n_{x,ij} \times n_{x,ij}}$ is an identity matrix. 

Note that the vector $e_{n}^k$ described in~\eqref{eq:SystemMatricesOfDelayFreePresentationSISO} becomes a matrix in the MIMO case, we thus rename it as $E_{n}^k$. Then we introduce a matrix 
\begin{equation}
    \bar{E}_h = \left [E_{m_{11}+h}^{\bar{m}+1}; E_{m_{21}+h}^{\bar{m}+1}; \ldots ; E_{m_{n_z n_u}+h}^{\bar{m}+1} \right],
\end{equation}
where $ h \in \set{m_{ij} + h \leq \bar{m}+1}$ and $\bar{m}=\text{max}\left( m \right)$ indicates the maximum integer time delay constant.

% The vector $e_{n}^k$ described in~\eqref{eq:SystemMatricesOfDelayFreePresentationSISO} 
% is a matrix in the MIMO case, we thus rename it as $E_{n}^k$. We then introduce a matrix $\bar{E}_h$ as
% \begin{equation}
%     \bar{E}_h = \text{diag} \left( \begin{bmatrix}
%         E_{m_{11}+h}^{\bar{m}+1} & E_{m_{21}+h}^{\bar{m}+1} & \cdots & E_{m_{n_z n_u}+h}^{\bar{m}+1}
%     \end{bmatrix}\right),
% \end{equation}
% where $ h \in \set{m_{ij} + h \leq \bar{m}+1}$ and $\bar{m}=\text{max}\left( m \right)$ indicates the maximum integer time delay constant.

% Note that the case $n_u=1$ and $n_z=1$, the SISO system matrices $A_c$, $B_c$, $C_c$, $D_c$ and other related parameters are identical to the MIMO case, e.g., time delay constants $m = \bar{m}$, $v=V$, and $e_j=1$, $e_{n}^k = E_{n}^k$, $e_{m+1}^{m+1}= \bar{E}_{1}$ and $e_{m}^{m+1}=\bar{E}_{2}$.

Consequently, we obtain the delay-free discrete-time representation of the MIMO time-delay system by augmenting the system with the historical inputs $u_{o,k} = [u_{k-\bar{m}}; u_{k-\bar{m}+1}; \ldots; u_{k-1}]$. The delay-free discrete-time system for the MIMO time-delay system has the same expressions as the SISO case described in~\eqref{eq:Deterministic-DiscreteTimeDelayStateSpaceSISO},~\eqref{eq:IAandIB} and \eqref{eq:SystemMatricesOfDelayFreePresentationSISO}. However, $D_o$ in the MIMO case is computed as 
\begin{align}
    D_o = \begin{bmatrix}
        \bar{D}_{c,1} \\ \bar{D}_{c,2} \\ \vdots \\ \bar{D}_{c, n_z}
    \end{bmatrix},
    \quad
    \bar{D}_{c,i} = \sum_{j=1}^{n_u} D_{c,ij} e_j E_{m_{ij}}^{\bar{m} + 1}.
\end{align}
Note that when $n_u=1$ and $n_z=1$, the time delay constants $m = \bar{m}$, $v=V$, $e_j=1$, and system parameters $e_{n}^k = E_{n}^k$, $e_{m+1}^{m+1}= \bar{E}_{1}$ and $e_{m}^{m+1}=\bar{E}_{2}$. Consequently, the SISO discrete-time system is identical to the MIMO case.
%% %%%%%%%%%%%%%%%%%%%%%%%%
\begin{prop}
\label{prop:DiscretizationofMIMOTimeDelaySystem}
The system of differential equations
\begin{subequations}
\label{eq:MIMOTimeDelaySystem:MatrixODEsystem}
\begin{alignat}{3}
    \dot A(t) &= A_c A(t), \qquad && A(0) = I, \\
    \dot A_v(t) &= V A_c A_v(t), \qquad && A_v(0) = I, \\ 
    \dot B_1(t) &= A(t) B_{1c}, \qquad && B_1(0) = 0, \\
    \dot B_2(t) &= A_v(t) \bar{B}_{2c}, \qquad && B_2(0) = 0,
\end{alignat}
\end{subequations}
where 
\begin{equation}
    B_{1c} = B_c \odot \bar{E}_{1}, \: B_{2c} = B_c \odot \bar{E}_2, \: \bar{B}_{2c} = V(B_{2c} - B_{1c}),
\end{equation}
may be used to compute ($A = A(T_s)$, $B_o=B_1(T_s)+B_2(T_s)$) for the discretization of the continuous-time time-delay system.  
% {\flushright \hfill $\blacksquare$}
\end{prop}
%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Deterministic linear-quadratic optimal control problem}
Consider the deterministic LQ-OCP governed by a time-delay system~\eqref{eq:Deterministic-ContinuousTimeDelayStateSpaceMIMO}
\begin{subequations}
\label{eq:Deterministic:ContinuousTime:LinearQuadraticOCP}
\begin{alignat}{5}
& \min_{x,u,z,\tilde z} \, &&\phi = \int_{t_0}^{t_0+T} l_c(\tilde z(t)) dt \\
& s.t. && x(t_0) = \hat x_0, \\
& && u(t) = u_k, \: t_k \leq t < t_{k+1}, \: k \in \mathcal{N}, \\
& && \dot x(t) = A_c x(t) + B_c u(t-\tau), t_0 \leq t < t_0+T, \\
& && z(t) = C_c x(t) + D_c u(t-\tau), t_0 \leq t < t_0+T, \\
& && \bar z(t) = \bar z_k, \: t_k \leq t < t_{k+1}, \: k \in \mathcal{N}, \\
& && \tilde z(t) = z(t) - \bar z(t), \: t_0 \leq t < t_0+T,
\end{alignat}
\end{subequations}
with the stage cost function
\begin{equation}
\begin{split}
    l_c(\tilde z(t)) &= \frac{1}{2} \norm{ W_z \tilde z(t)  }_2^2
    = \frac{1}{2} \tilde z(t) ' Q_{c} \tilde z(t), 
\end{split}
\label{eq:det-stagecost}
\end{equation}
where the weight matrix $Q_c=W_z' W_z$ is semi-positive definite. $T = N T_s$ and $N \in \mathbb{Z}^+$ for $\mathcal{N} = 0, 1, \ldots, N-1$ is the control interval. We assume piece-wise constant inputs $u(t) = u_k$ and target variables $\bar z(t) = \bar{z}_k$ for $t_k \leq t < t_{k+1}$. 

% and $Q_{c} = W_z' W_z$ is a semi-positive definite matrix. This problem is in continuous-time with decision variables $x(t),u(t),z(t),\Tilde{z}(t)$. The control interval $T = N T_s$ with $N \in \mathbb{Z}^+$, and $\mathcal{N} = 0, 1, \ldots, N-1$. We assume piecewise constant inputs $u(t) = u_k$ and target variables $\bar z(t) = \bar{z}_k$ for $t_k \leq t < t_{k+1}$. 

The corresponding discrete-time LQ-OCP is
\begin{subequations}
\label{eq:Deterministic:DiscreteTime:LinearQuadraticOCP}
\begin{alignat}{5}
& \min_{x,u} \quad &&\phi = \sum_{k\in \mathcal{N}} l_k(x_k,u_k)  \\
& s.t. && x_0 = \hat x_0, \\
& && x_{k+1} = A x_k + B u_k, \quad && k \in \mathcal{N},
\end{alignat}    
\end{subequations}
where the states $x$ and system matrices $A$, $B$, $C$, $D$ are in the augmented form described in~\eqref{eq:Deterministic-DiscreteTimeDelayStateSpaceSISO}. The stage cost function $l_k(x_k, u_k)$ is 
\begin{equation}
    l_k(x_k,u_k) = \frac{1}{2} \begin{bmatrix} x_k \\ u_k \end{bmatrix}' Q \begin{bmatrix} x_k \\ u_k \end{bmatrix} + q_k' \begin{bmatrix} x_k \\ u_k \end{bmatrix} + \rho_k, \quad k \in \mathcal{N},
\label{eq:deterministic-stageCost}
\end{equation}
and its affine term's coefficients and the constant term are 
\begin{equation}
    q_k =  M \bar{z}_k, \:  \rho_k =  \int_{t_k}^{t_{k+1}} l_c(\bar{z}_k) dt = l_c(\bar z_k) T_s, \: k \in \mathcal{N}.
\label{eq:qkandrho_k}
\end{equation}
% The state vector $x$ and system matrices $A$, $B$, $C$, $D$ are in the augmented form described in~\eqref{eq:Deterministic-DiscreteTimeDelayStateSpaceSISO}. The coefficient in the affine term and the constant term are
% \begin{equation}
%     q_k =  M \bar{z}_k, \:  \rho_k =  \int_{t_k}^{t_{k+1}} l_c(\bar{z}_k) dt = l_c(\bar z_k) T_s, \: k \in \mathcal{N}.
% \label{eq:qkandrho_k}
% \end{equation}
%
\begin{prop} The system of differential equations
\label{prop:DiscretizationoftheDterministicLQOCP}
\begin{subequations}
\label{eq:DeterministicLQ:MatrixODEsystem}
\begin{alignat}{3}
    \dot A(t) &= A_c A(t), \qquad && A(0) = I, \\
    \dot A_v(t) &= VA_c A_n(t), \qquad && A_v(0) = I, \\
    \dot B_1(t) &=  A(t)  B_{1c}, \qquad && B_1(0) = 0, \\
    \dot B_2(t) &= A_v(t) \bar B_{2c}, \qquad && B_2(0) = 0, \\
    \dot Q(t) &= \Gamma(t)'  Q_{c} \Gamma(t), \qquad && Q(0) = 0,  \\
    \dot M(t) &= -\Gamma(t)' M_{c}, \qquad && M(0) = 0,
\end{alignat}
\end{subequations}
where
\begin{subequations}
\begin{equation}
   B_{1c} = B_c \odot \bar{E}_{1}, B_{2c} = B_c \odot \bar{E}_2, \bar{B}_{2c} = V(B_{2c} - B_{1c}),
\end{equation}
% \begin{equation}
%     H_c = \begin{bmatrix} C_c & D_o \end{bmatrix}, 
%     \quad 
%     \bar M_c = -H_c' Q_c, 
%     \quad
%     \bar Q_c = - \bar M_c H_c,
% \end{equation}
\begin{equation}
    \Gamma(t) = \begin{bmatrix} C_c & D_o \end{bmatrix} \begin{bmatrix} A(t) & B_o(t) \\ 0 & I \end{bmatrix}, 
\end{equation}
\end{subequations}
may be used to compute ($A = A(T_s)$, $B_o=B_1(T_s)+B_2(T_s)$, $Q=Q(T_s)$, $M=M(T_s)$) for the discretization of the deterministic LQ-OCP. 
% {\flushright \hfill $\blacksquare$}
\end{prop}
%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Certainty equivalent LQ control for a stochastic time-delay system}
Consider a continuous-time linear stochastic differential equations (SDEs) system with time delays
\begin{subequations}
\label{eq:linearSDE}
\begin{alignat}{3}
    d {\bs x}(t) &= \left( A_c {\bs x}(t) + B_c u(t-\tau) \right) dt + G_c d{\bs \omega}(t), \\
    {\bs z}(t) &= C_c {\bs x}(t) + D_c  u(t-\tau).
\end{alignat}
\end{subequations}
where the state $\bs x$ and stochastic variable $\bs \omega$ are
\begin{align}
    {\bs x}(t_0) & \sim N(\hat x_0,P_0), \qquad 
    d{\bs \omega} (t) \sim N_{iid}(0, I dt).
\end{align}
The corresponding delay-free discrete-time representation of the linear time-delay SDEs is 
\begin{subequations}
\label{eq:Stochastic-DiscreteTimeDelayStateSpaceMIMO}%
\begin{alignat}{3}
    \Tilde{\bs x}_{k+1} &= \Tilde{A} \Tilde{\bs x}_k + \Tilde{B} u_k + \Tilde{\bs w}_k, \\
    {\bs z}_k &= \Tilde{C} \Tilde{\bs x}_k +  \Tilde{D} u_k,
\end{alignat} 
\end{subequations}
where $\Tilde{A}$, $\Tilde{B}$, $\Tilde{C}$ and $\Tilde{D}$ are identical to the deterministic case~\eqref{eq:Deterministic-DiscreteTimeDelayStateSpaceSISO}. The state $\Tilde{\bs x} = \left[ \bs x; u_o \right]$ and 
\begin{subequations} 
\label{eq:augmentedStateAndStochastics}%
\begin{equation}
    \Tilde{\bs x} \sim N \left( \Tilde{x}_0, \Tilde{P}_0 \right), \quad 
    \Tilde{x}_0 = \begin{bmatrix} x_0 \\ u_{o,0} \end{bmatrix}, \quad 
    \Tilde{P}_0 = \begin{bmatrix} P_0 & 0 \\ 0 & 0  \end{bmatrix},
\end{equation}
and the stochastic variable $\Tilde{\bs w}$ is
\begin{equation}
    \Tilde{\bs w} = \begin{bmatrix} \bs w \\ 0 \end{bmatrix} \sim N_{iid} \left( 0, \Tilde{R}_{ww} \right), \quad 
    \Tilde{R}_{ww} = \begin{bmatrix} R_{ww} & 0 \\ 0 & 0  \end{bmatrix}.
\end{equation}
\end{subequations}
% 
\begin{prop}
\label{prop:DiscretizationoftheLinearSDE}
The system of differential equations
\begin{subequations}
\begin{alignat}{3}
    \dot A(t) &= A_c A(t), \qquad && A(0) = I, \\
    \dot A_v(t) &= V A_c A_v(t), \qquad && A_v(0) = I, \\ 
    \dot B_1(t) &= A(t) B_{1c}, \qquad && B_1(0) = 0, \\
    \dot B_2(t) &= A_v(t) \bar{B}_{2c}, \qquad && B_2(0) = 0, \\
    \dot R_{ww} &= \Phi(t) \Phi(t)', \qquad && R_{ww}(0) = 0,
\end{alignat}
\end{subequations}
where 
\begin{subequations}
\begin{alignat}{3}
    & B_{1c} = B_c \odot \bar{E}_{1}, \qquad && B_{2c} = B_c \odot \bar{E}_2, \\
    & \bar{B}_{2c} = V(B_{2c} - B_{1c}), \qquad  && \Phi(t) = A(t) G_c,
\end{alignat}
\end{subequations}
may be used to compute ($A=A(T_s)$, $B_o=B_1(T_s)+B_2(T_s)$, $R_{ww}=R_{ww}(T_s)$) for the discretization of the stochastic time-delay system.
% {\flushright \hfill $\blacksquare$}
\end{prop}
%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Stochastic linear-quadratic optimal control problem}
Consider the stochastic LQ-OCP governed by the stochastic time-delay system~\eqref{eq:linearSDE}
\begin{subequations}
\label{eq:Cont-Stc-LQ-OCP}
\begin{alignat}{5}
& \min_{{\bs x},u,{\bs z},{\tilde{\bs z}}} \: \psi = E \set{ \phi = \int_{t_0}^{t_0+T} l_c({\tilde{\bs z}}(t))dt }  \MoveEqLeft[1] \\
&  s.t. \quad  {\bs x}(t_0) \sim N(\hat x_0, P_0), \\
&  \qquad \: d{\bs \omega}(t) \sim N_{iid}(0,I dt), \\
&  \qquad \: u(t) = u_k, \quad t_k \leq t < t_{k+1}, \, k \in \mathcal{N}, \\
& \qquad \: d{\bs x}  (t) = (A_c {\bs x}(t) + B_c u(t-\tau))dt + G_c d{\bs \omega}(t), \\
& \qquad \: {\bs z}(t) = C_c {\bs x}(t) + D_c u(t-\tau), \\
& \qquad \: {\bar z}(t) = \bar z_k, \quad t_k \leq t < t_{k+1}, \, k \in \mathcal{N}, \\
& \qquad \: {\tilde {\bs z}}(t) = {\bs z}(t) - \bar{z}(t).
\end{alignat}
\end{subequations}
The corresponding discrete-time stochastic LQ-OCP is 
\begin{subequations}
\label{eq:Dist-Stc-LQ-OCP}
\begin{alignat}{5}
& \min_{ x,u} \quad  && \psi = E\set{\phi = \sum_{k \in \mathcal{N}} l_k({\bs x}_k,u_k) + l_{s,k} (\bs{x}_k,u_k)}  \\ 
& s.t. && {\bs x}_0 \sim N(\hat x_0, P_0), \\
& && {\bs w_k} \sim N_{iid}(0,R_{ww}), \qquad \qquad k \in \mathcal{N}, \\
& && {\bs x}_{k+1} = A {\bs x}_k + B u_k + {\bs w}_k, \quad \: k \in \mathcal{N}, 
\end{alignat}
\end{subequations}
where the state $\bs x_k$ and stochastic variable $\bs w_k$, and the system matrices $A$, $B$, $C$, $D$ are in the augmented form described in~\eqref{eq:Stochastic-DiscreteTimeDelayStateSpaceMIMO} and~\eqref{eq:augmentedStateAndStochastics}. The stage cost function $l_k(\bs{x}_k, u_k)$ 
\begin{equation}
l_k(\bs{x}_k,u_k) = \frac{1}{2} \begin{bmatrix} \bs{x}_k \\ u_k \end{bmatrix}' Q \begin{bmatrix} \bs{x}_k \\ u_k \end{bmatrix} + q_k' \begin{bmatrix} \bs{x}_k \\ u_k \end{bmatrix} + \rho_k,
\label{eq:deterministicStageCostofStochasticCosts}
\end{equation}
and $l_{s,k}(\bs{x}_k, u_k)$ 
\begin{equation}
    l_{s,k}(\bs{x}_k, u_k) = \int_{t_k}^{t_{k+1}} \frac{1}{2} \bs{w}(t)' Q_{c,ww} \bs{w}(t) + \bs{q}_{s,k}' \bs{w}(t) dt.
\end{equation}
where $Q$, $q_k$, and $\rho_k$ are identical to the deterministic case described in~\eqref{eq:qkandrho_k} and~\eqref{eq:DeterministicLQ:MatrixODEsystem}. The state $\bs w(t)$ and system matrices $Q_{c,ww}$ and $\bs q_{s,k}$ of $l_{s,k}(\bs{x}_k,u_k)$ are
\begin{subequations}
    \begin{align}
        & \bs{w}(t) = \int_{0}^{t} A(s) G_c d\bs{\omega}(s),  \quad 
        && Q_{c,ww} = C_c' Q_{c} C_c,  
        \\
        & \Tilde{\bs{z}}_k = \Gamma(t) \begin{bmatrix} \bs{x}_k \\ u_k \end{bmatrix} - \bar{z}_k, 
        && \bs{q}_{s,k} = C' Q_{c} \Tilde{\bs{z}}_k.
    \end{align}
\end{subequations}
Based on the previous work by~\cite{Karl1970IntroToStoContTheory}, we can rewrite~\eqref{eq:Dist-Stc-LQ-OCP} as
\begin{subequations} 
\label{eq:analyticMeanOfStochasticCosts01}
\begin{alignat}{5}
& \min_{ x,u } \: && \psi = \sum_{k \in \mathcal{N}} l_k(x_k,u_k) + \bs \rho_{s,k}\\
& s.t. && x_0 = \hat x_0, \\
& &&  x_{k+1} = A x_k + B u_k, \quad k \in \mathcal{N}, 
\end{alignat}
\end{subequations}
where $\bs \rho_{s,k}$ is 
\begin{subequations} \label{eq:analyticMeanOfStochasticCosts02}
    \begin{equation}
        \bs \rho_{s,k} = \frac{1}{2} \left[ \text{tr}\left( Q \bar{P}_k \right) + \int_{t_k}^{t_{k+1}} \text{tr} \left(Q_{c,ww} P_{w} \right) dt \right],
    \end{equation}
and $ $
    \begin{equation}
    \begin{bmatrix}
            \bs{x}_k \\ u_k
        \end{bmatrix} \sim N(m_k, \bar{P}_k),
    \: 
    m_k = \begin{bmatrix}
        x_k \\ u_k
    \end{bmatrix},
    \: 
    \bar{P}_k = \begin{bmatrix} P_k & 0 \\ 0 & 0 \end{bmatrix},
\end{equation}
    %
\begin{equation}
    P_{k+1} = A P_k A' + R_{ww}, \qquad P_w = \text{Cov} \left(\bs{w}(t)\right).
\end{equation}
\end{subequations}
%% %%%%%%%%%%%%%%%%%%%%%%%%%
\begin{prop}
\label{prop:DiscretizationoftheStochasticLQ-OCP}
The system of differential equations
\begin{subequations}
\label{eq:StochasticLQG:MatrixODEsystem}
\begin{alignat}{3}
    \dot A(t) &= A_c A(t), \qquad && A(0) = I, \\
    \dot A_v(t) &= V A_c A_v(t), \qquad && A_v(0) = I, \\ 
    \dot B_1(t) &= A(t) B_{1c}, \qquad && B_1(0) = 0, \\
    \dot B_2(t) &= A_v(t) \bar{B}_{2c}, \qquad && B_2(0) = 0, \\
    \dot Q(t) &= \Gamma(t)' Q_{c} \Gamma(t), \qquad && Q(0) = 0,  \\
    \dot M(t) &= -\Gamma(t)' Q_{c}, \qquad && M(0) = 0, \\
    \dot R_{ww}(t) &= \Phi(t) \Phi(t)', \qquad && R_{ww}(0) = 0, 
\end{alignat}
\end{subequations}
where 
\begin{subequations}
\begin{equation}
        B_{1c} = B_c \odot \bar{E}_{1}, B_{2c} = B_c \odot \bar{E}_2, \bar{B}_{2c} = V(B_{2c} - B_{1c}),
\end{equation}
\begin{equation}
    \Gamma(t) = \begin{bmatrix} C_c & D_o \end{bmatrix} \begin{bmatrix} A(t) & B_o(t) \\ 0 & I \end{bmatrix}, \qquad 
    \Phi(t) = A(t)G_c,
\end{equation}
\end{subequations}
may be used to compute ($A=A(T_s)$, $B_o=B_1(T_s)+B_2(T_s)$, $Q=Q(T_s)$, $M=M(T_s)$, $R_{ww}=R_{ww}(T_s)$) for the discretization of the stochastic LQ-OCP with time delays.
% {\flushright \hfill $\blacksquare$}
\end{prop}
%%
